hidden markov random fields and cuckoo search method for medical image segmentation

Segmentation of medical images is an essential part in the process of diagnostics. Physicians require an automatic, robust and valid results. Hidden Markov Random Fields (HMRF) provide powerful model. This latter models the segmentation problem as the minimization of an energy function. Cuckoo search (CS) algorithm is one of the recent nature-inspired meta-heuristic algorithms. It has shown its efficiency in many engineering optimization problems. In this paper, we use three cuckoo search algorithm to achieve medical image segmentation.

==> HMRF-CS #2/file <==
a rajouter dans Intro
Cuckoo search algorithm was developed by Yang and Deb in 2009 which is instigated by the coerce brood parasitism of some cuckoo species by laying their eggs in 
the nests of other host birds. Some host birds can slot in unswerving clash with the obtrusive cuckoos. For example, 
if a host bird discovers the eggs that are not their own, it can neither throw these unfamiliar eggs nor leave the nest 
and erect up a new one. In some cuckoo species the female cuckoos are experts in the parody in colors and pattern of the eggs in certain host species. Cuckoo search has idealized such breeding behavior and so can be applied to a wide range of optimization problems. CS surpasses the other meta-heuristic algorithms in relevance.

Discovery rate of alien eggs/solutions

$\mu^{i,t+1}=(\mu^{i,t+1}_1,,\dots,\mu^{i,t+1}_j,\dots,\mu^{i,t+1}_K)$


==> file <==
a rajouter dans Intro
Cuckoo search algorithm was developed by Yang and Deb in 2009 which is instigated by the coerce brood parasitism of some cuckoo species by laying their eggs in 
the nests of other host birds. Some host birds can slot in unswerving clash with the obtrusive cuckoos. For example, 
if a host bird discovers the eggs that are not their own, it can neither throw these unfamiliar eggs nor leave the nest 
and erect up a new one. In some cuckoo species the female cuckoos are experts in the parody in colors and pattern of the eggs in certain host species. Cuckoo search has idealized such breeding behavior and so can be applied to a wide range of optimization problems. CS surpasses the other meta-heuristic algorithms in relevance.

Discovery rate of alien eggs/solutions

$\mu^{i,t+1}=(\mu^{i,t+1}_1,,\dots,\mu^{i,t+1}_j,\dots,\mu^{i,t+1}_K)$

